Mesh-free Eulerian Physics-Informed Neural Networks

Physics-informed Neural Networks (PINNs) have recently emerged as a principled way to include prior physical knowledge in form of partial differential equations (PDEs) into neural networks. Although PINNs are generally viewed as mesh-free, current approaches still rely on collocation points within a bounded region, even in settings with spatially sparse signals. Furthermore, if the boundaries are not known, the selection of such a region is difficult and often results in a large proportion of collocation points being selected in areas of low relevance. To resolve this severe drawback of current methods, we present a mesh-free and adaptive approach termed particle-density PINN (pdPINN), which is inspired by the microscopic viewpoint of fluid dynamics. The method is based on the Eulerian formulation and, different from classical mesh-free method, does not require the introduction of Lagrangian updates. We propose to sample directly from the distribution over the particle positions, eliminating the need to introduce boundaries while adaptively focusing on the most relevant regions. This is achieved by interpreting a non-negative physical quantity (such as the density or temperature) as an unnormalized probability distribution from which we sample with dynamic Monte Carlo methods. The proposed method leads to higher sample efficiency and improved performance of PINNs. These advantages are demonstrated on various experiments based on the continuity equations, Fokker-Planck equations, and the heat equation.

==> subfiles/08_checklist.tex <==

%%% BEGIN INSTRUCTIONS %%%
% The checklist follows the references.  Please
% read the checklist guidelines carefully for information on how to answer these
% questions.  For each question, change the default \answerTODO{} to \answerYes{},
% \answerNo{}, or \answerNA{}.  You are strongly encouraged to include a {\bf
% justification to your answer}, either by referencing the appropriate section of
% your paper or providing a brief inline description.  For example:
% \begin{itemize}
%   \item Did you include the license to the code and datasets? \answerYes{See Section~\ref{gen_inst}.}
%   \item Did you include the license to the code and datasets? \answerNo{The code and the data are proprietary.}
%   \item Did you include the license to the code and datasets? \answerNA{}
% \end{itemize}
% Please do not modify the questions and only use the provided macros for your
% answers.  Note that the Checklist section does not count towards the page
% limit.  In your paper, please delete this instructions block and only keep the
% Checklist section heading above along with the questions/answers below.
%%% END INSTRUCTIONS %%%


\begin{enumerate}
\item For all authors...
\begin{enumerate}
  \item Do the main claims made in the abstract and introduction accurately reflect the paper's contributions and scope?
    \answerYes{}
  \item Did you describe the limitations of your work?
    \answerYes{See Conclusions section~\ref{sec:conclusion}.}
  \item Did you discuss any potential negative societal impacts of your work?
    \answerNA{Our work has a theoretical focus in the context of physics-informed neural networks without a clear relationship to societal aspects.}
  \item Have you read the ethics review guidelines and ensured that your paper conforms to them?
    \answerYes{}
\end{enumerate}


\item If you are including theoretical results...
\begin{enumerate}
  \item Did you state the full set of assumptions of all theoretical results?
    \answerYes{We state assumptions and requirements for our approach to hold.}
        \item Did you include complete proofs of all theoretical results?
    \answerNA{We do not state theorems or propositions and thus do not provide proofs.}
\end{enumerate}


\item If you ran experiments...
\begin{enumerate}
  \item Did you include the code, data, and instructions needed to reproduce the main experimental results (either in the supplemental material or as a URL)?
    \answerYes{See appendix.}
  \item Did you specify all the training details (e.g., data splits, hyperparameters, how they were chosen)?
    \answerYes{See appendix.}
  \item Did you report error bars (e.g., with respect to the random seed after running experiments multiple times)?
    \answerYes{All results are obtained for different random seeds and box plots are provided.}
  \item Did you include the total amount of compute and the type of resources used (e.g., type of GPUs, internal cluster, or cloud provider)?
    \answerYes{See appendix.}
\end{enumerate}


\item If you are using existing assets (e.g., code, data, models) or curating/releasing new assets...
\begin{enumerate}
  \item If your work uses existing assets, did you cite the creators?
    \answerYes{We cited original work which we used in our experiments or as a basis for our approach, as for example SIREN or relevant related approaches.}
  \item Did you mention the license of the assets?
    \answerNA{No license involved in using established neural network architectures.}
  \item Did you include any new assets either in the supplemental material or as a URL?
    \answerNA{Does not apply.}
  \item Did you discuss whether and how consent was obtained from people whose data you're using/curating?
    \answerNA{Does not apply; we relied only on simulations of the data.}
  \item Did you discuss whether the data you are using/curating contains personally identifiable information or offensive content?
    \answerNA{Does not apply, for the same reason as in the previous point.}
\end{enumerate}


\item If you used crowdsourcing or conducted research with human subjects...
\begin{enumerate}
  \item Did you include the full text of instructions given to participants and screenshots, if applicable?
    \answerNA{No human subjects involved, only physics simulations were considered.}
  \item Did you describe any potential participant risks, with links to Institutional Review Board (IRB) approvals, if applicable?
    \answerNA{Does not apply.}
  \item Did you include the estimated hourly wage paid to participants and the total amount spent on participant compensation?
    \answerNA{Does not apply.}
\end{enumerate}


\end{enumerate}

==> subfiles/09_tables.tex <==
%
\begin{table}[h]
\begin{center}
\begin{tabular}{llllllll}
\caption{ Test $R^2$ of $\sqrt{\rho}$, for varying number of collocation
points}
\label{table:exp_3d_opt}
	%\toprule
	 & & \multicolumn{3}{c}{Avg $R^2$ of $\sqrt{\rho}\ \ $  ($\pm std$)} \\
	 \midrule
	 \# collocation points &                  256   &&               4096  &&               65536 \\
	\midrule
	Baseline            &0.62 &($\pm$0.013)&0.62 &($\pm$0.013)&0.62 &($\pm$0.013)\\
	Uniform             &   0.622 &($\pm$0.01) &  0.639 &($\pm$0.012) &  0.743 &($\pm$0.012) \\
	RAR                 &  0.625 &($\pm$0.011) &   0.64 &($\pm$0.013) &  0.756 &($\pm$0.015) \\
	OT-RAR              &   0.627 &($\pm$0.01) &  0.665 &($\pm$0.021) &   0.763 &($\pm$0.01) \\
	importance-sampling &  0.658 &($\pm$0.019) &  0.716 &($\pm$0.022) &  0.725 &($\pm$0.038) \\
	IT-pdPINN           &  0.693 &($\pm$0.024) &  0.737 &($\pm$0.029) &  0.751 &($\pm$0.039) \\
	MH-pdPINN           &  \textbf{0.699}&($\pm$0.018) &  \textbf{0.743}&($\pm$0.034) &  \textbf{0.77} &($\pm$0.007) \\
	\bottomrule
\end{tabular}
\end{center}
\end{table}
%
